Powers of Hamilton cycles in random graphs and tight Hamilton cycles in random hypergraphs

We show that for every $k \in \mathbb{N}$ there exists $C > 0$ such that if $p^k \ge C \log^8 n / n$ then asymptotically almost surely the random graph $G_{n,p}$ contains the $k$\textsuperscript{th} power of a Hamilton cycle. This determines the threshold for appearance of the square of a Hamilton cycle up to the logarithmic factor, improving a result of K\"uhn and Osthus. Moreover, our proof provides a randomized quasi-polynomial algorithm for finding such powers of cycles. Using similar ideas, we also give a randomized quasi-polynomial algorithm for finding a tight Hamilton cycle in the random $k$-uniform hypergraph $G_{n,p}^{(k)}$ for $p \ge C \log^8 n/ n$. The proofs are based on the absorbing method and follow the strategy of K\"uhn and Osthus, and Allen et al. The new ingredient is a general Connecting Lemma which allows us to connect tuples of vertices using arbitrary structures at a nearly optimal value of $p$. Both the Connecting Lemma and its proof, which is based on Janson's inequality and a greedy embedding strategy, might be of independent interest.

==> tools.tex <==
%!TEX root = square_hamilton.tex
\section{Blah} \label{sec:preliminaries}

We use lower tail estimates for random
variables which count the number of copies of certain graphs in a
random graph. The following version of
Janson's inequality, tailored for graphs, will suffice. The
statement follows immediately from Theorems $8.1.1$ and $8.1.2$ in
\cite{alon2004probabilistic}.

\begin{theorem}[Janson's inequality] \label{thm:Janson}
Let $p \in (0, 1]$ and consider a family $\{ H_i \}_{i \in
\mathcal{I}}$ of subgraphs of the complete graph on the vertex set
$[n]$. Let $G \sim \Gnp$ and, for each $i \in \mathcal{I}$, let $X_i$
denote the indicator random variable for the event that $H_i \subseteq
G$ and, for each ordered pair $(i, j) \in \mathcal{I} \times
\mathcal{I}$ with $i \neq j$, write $H_i \sim H_j$ if $E(H_i)\cap
E(H_j)\neq \emptyset$. Then, for
\begin{align*}
X &= \sum_{i \in \mathcal{I}} X_i, \\
\mu &= \mathbb{E}[X] = \sum_{i \in \mathcal{I}} p^{e(H_i)}, \\
\delta &= \sum_{\substack{(i, j) \in \mathcal{I} \times \mathcal{I} \\ H_i \sim H_j}} \mathbb{E}[X_i X_j] = \sum_{\substack{(i, j) \in \mathcal{I} \times \mathcal{I} \\ H_i \sim H_j}} p^{e(H_i) + e(H_j) - e(H_i \cap H_j)}
\end{align*}
and any $0 < \gamma < 1$, we have
$$ \Pr[X < (1 - \gamma)\mu] \le e^{- \frac{\gamma^2 \mu^2}{2(\mu + \delta)}}. $$
\end{theorem}


\subsection{Large $F$-matchings in random graphs}

Given graphs $H$ and $G$ and a real $\varepsilon \ge 0$, we say that $G$ contains an \emph{$(H, \varepsilon)$-factor} if there exists a family of vertex-disjoint copies of $H$ in $G$ covering all but at most $\varepsilon v(G)$ vertices of $G$. The case $\varepsilon = 0$ is usually referred to as an $H$-factor, and (a small) $\varepsilon > 0$ as an \emph{almost} $H$-factor. For a fixed graph $H$, finding the correct order of magnitude of $p$ for which $\Gnp$ contains an $H$-factor has received a lot of attention until it was finally resolved by Johansson, Kahn and Vu \cite{JoKaVu08} (albeit only for balanced graphs). Based on an earlier result on $H$-factors by Alon and Yuster \cite{AlYu97}, the case $H = H(n)$ (i.e. $H$ is not a fixed graph but rather an infinite sequence of growing graphs $(H_n)_{n \in \mathbb{N}}$) and $\varepsilon = 0$ was studied in \cite{YaWaHa08}. Their result imposes certain structural properties on $H_n$, and, more importantly, an upper-bound $v(H_n) = o(\sqrt{\log n})$ on the size of $H_n$. Such a bound, however, does not work for us as in Section \ref{sec:absorbers} we aim to find an $(H,\eps)$-factor with $v(H) = \Theta(\log^2 n)$. Here we give a simple argument based on Janson's inequality in the case where $\varepsilon > 0$ and $H$ has $o(n^{1/4})$ vertices. We use the notion of $m_1$-density of a (hyper)graph $G$, %denoted by $m_1(G)$ and 
 defined as 
$$
m_1(G) = \max\left\{ \frac{e(H)}{v(H) - 1} \; : \; H \subseteq G \text{ and } e(H) \ge 1\right\}.
$$

\begin{lemma} \label{lemma:manycopies}
Given an integer $k \ge 2$ and reals $\varepsilon > 0$ and $\beta > 1$, there exist $C > 0$ and $n_0 \in \mathbb{N}$ such that the following holds: for every $n \ge n_0$ and a $k$-graph $H$ on at most $(n / C)^{1/4}$ vertices, if 
$$
	p \ge \left( \frac{C v(H)^4}{n} \right)^{1/m_1(H)}
$$
then $\Gknp$ contains an $(H, \varepsilon)$-factor with probabiliity at least $1 - e^{- \beta n}$. Moreover, there is an $n^{O(v(H))}$ algorithm for finding such a factor.
\end{lemma}

Lemma \ref{lemma:manycopies} follows easily from a union-bound and the following claim which gives an upper bound on the probability that a random hypergraph on $n$ vertices does not contain a given subgraph $H$. %Moreover, Lemma \ref{lemma:m_1} is suitable  even when $H$ has a size growing with $n$. The proof is a straightforward application of Janson's inequality, thus we defer it for the appendix.

\begin{claim} \label{claim:m_1}
For every integer $k \ge 2$ and a real $\beta > 1$, there exist constants $C > 0$ and $n_0 \in \mathbb{N}$ such that the following holds: for every $n \ge n_0$ and a $k$-graph $H$ on at most $(n/C)^{1/4}$ vertices, if
$$
	p \ge \left( \frac{C v(H)^4}{n} \right)^{1/m_1(H)}
$$
then $G \sim \mathcal{G}^{(k)}(n, p)$ contains $H$ with probability at least $1 - e^{-\beta n}$.
\end{claim}

Having Claim \ref{claim:m_1} at hand, we derive Lemma \ref{lemma:manycopies}.

\begin{proof}[Proof of Lemma \ref{lemma:manycopies}]
Let $C'$ be a constant given by Claim \ref{claim:m_1} for $\beta + 1$ (as $\beta$). We show the lemma for $C = C' / \eps$. First, note that for a subset $V' \subseteq V(G)$ of size $|V'| = \eps n$ we have $G[V'] \sim \mathcal{G}^{(k)}(\eps n, p)$ thus, as $p \ge (C' v(H)^4 / \eps n)^{1/m_1(H)}$, $G[V']$ contains $H$ with probability at least $1 - e^{-(\beta + 1)n}$ (Claim \ref{claim:m_1}). As there are at most $2^n$ subsets $V' \subseteq V(G)$ of size $\eps n$, by a simple union bound we conclude that $G[V']$ contains $H$ for all such subsets with probability at least $1 - e^{\beta n}$. This property gives an easy greedy algorithm for constructing an $(H, \eps)$-factor in time $n^{O(v(H)}$: let $U := V(G)$ and as long as $|U| \ge \eps n$ choose an arbitrary subset $V' \subseteq U$ of size $\eps n$, find a copy of $H$ in $G[V']$ and remove its vertices from $U$. Each such copy of $H$ can be found in $n^{O(v(H))}$ time by simply trying all possible permutations of each subset of $v(H)$ vertices.
\end{proof}

Finally, it remains to prove Claim \ref{claim:m_1}.

\begin{proof}[Proof of Claim \ref{claim:m_1}]
We show a lower bound on the desired event by using Janson's inequality. Let $V(H) = \{u_1, \ldots, u_{v(H)}\}$ be a labeling of the vertices of $H$ and let $\mathcal H$ denotes the family of all \emph{lexicographical} copies of $H$ in $K_n$, i.e. a family of subgraphs $\hat H \subseteq K^{(k)}_n$ with $v(H)$ vertices such that the unique bijection $f \colon V(H) \to V(\hat H)$ satisfying  
$$
f(u_j) < f(u_{j+1}),\text{ for all } 1 \le j < v(H)
$$
is an isomorphism between $H$ and $\hat H$. We implicitly assume that $K_n^{(k)}$ is a complete $k$-graph on the vertex set $[n]$. Since every choice of $v(H)$ vertices from $K^{(k)}_n$ uniquely determines a lexicographical copy of $H$ we have $|\mathcal{H}| = \binom{n}{v(H)}$. Therefore, the expected number of $\hat H \in \mathcal H$ that appear in $G$ is
$$
\mu = |\mathcal H| p^{e(H)} = \binom{n}{v(H)} p^{e(H)}.
$$
Note that as $e(H) \le (v(H) -1) m_1(H)$ we can lower bound $\mu$ as follows,
$$
\mu \ge \left (\frac{n}{v(H)} \right)^{v(H)} p^{(v(H)-1) m_1(H)} \ge \left(\frac{n}{v(H)} \right)^{v(H)} \left( \frac{C v(H)^4}{n} \right)^{v(H)-1} \ge C v(H)^{3v(H) - 4} n > C n,
$$
assuming that $V(H) > 1$.

As we aim to apply Janson's inequality to deduce that the probability of no $\hat H \in \mathcal H$ appearing in $G$ is sufficiently small, we now estimate the parameter $\delta$ as defined in Theorem \ref{thm:Janson},
$$
	\delta = \sum_{H' \sim H''}^{\mathcal H} p^{2e(H) - e(H' \cap H'')}.
$$
We use the above notation $\sum^{\mathcal{H}}$ to indicate that $H', H'' \in \mathcal{H}$. Since we are dealing with lexicographic copies, once we know the vertices of $H'$ and $H''$ both graphs are uniquely determined. Thus, we choose $H'$ and $H''$ by first fixing the number $j$ of vertices in their intersection, then picking $j$ vertices from $K_n^{(k)}$ for the intersection and finally picking two sets of $v(H)-j$ vertices to complete $H'$ and $H''$. Note that by choosing the copies in this way we do not have the control over the exact number of edges in their intersection. However, as the intersection is  a subgraph of $H$ we know that there can be at most $(j-1)m_1(H)$ many edges in $E(H') \cap E(H'')$. Following this counting strategy and using simple algebraical manipulation we obtain the following estimate on $\delta$,
\begin{align*}
\delta & \le \sum_{j = k}^{v(H)-1} \binom{n}{j} \binom{n-j}{v(H)-j}^2 p^{2e(H) -  (j-1)m_1(H) } \\ 
& =  \sum_{j = k}^{v(H)-1} \binom{n}{j} \left ( \binom{n}{v(H)} \binom{v(H)}{j} \binom{n}{j}^{-1} \right)^2 p^{2e(H) -  (j-1)m_1(H) } \\
& =  \mu^2 \sum_{j = k}^{v(H)-1} \binom{n}{j}^{-1}  \binom{v(H)}{j}^2  p^{-  (j-1)m_1(H) }, 
\end{align*}
where we used $\mu = \binom{n}{v(H)}p^{e(H)}$ in the last step.
Next, using standard binomial coefficient estimates and the lower bound on $p$ we get
\begin{align*}
\delta &\le \mu^2 \sum_{j = k}^{v(H) - 1} \left( \frac{e^2 v(H)^2}{j n} \right)^j 
\left( \frac{C v(H)^4}{n} \right)^{-(j-1)}
%& \le \frac\mu^2 \sum_{j = k}^{v(H)} \left( \frac{8 v(H)^2}{j n} \right)^j 
%v(H)^{-4(j-1)}  \cdot n^{j-1} C^{-(j-1)m_1(H)} \\
\le \frac{\mu^2}{n} \sum_{j = k}^{v(H) - 1} \left( \frac{e^2 v(H)^2}{j} \right)^j \left( \frac{1}{C v(H)^4} \right)^{j-1}
\\
& \le \frac{\mu^2}{n} \sum_{j = k}^{v(H) - 1} \left( e^4 v(H)^4 \right)^{j-1} \left( \frac{1}{C v(H)^4} \right)^{j-1} \le \frac{\mu^2}{n} \sum_{j = k}^{v(H) - 1} \left( e^4 / C \right)^{j-1} \le \frac{\mu^2}{C' n}.
\end{align*}
In the last step we used the fact that $\sum_{j = k}^{v(H)} \left( e^4/C \right)^{j-1}$ is a geometric sum thus for every $C' > 1$ there exists such $C = C(C')$.

Finally, let $X$ is the number of lexicographic copies $\hat H \in \mathcal{H}$ that appear in $G$. For a given $\beta > 0$ and sufficiently large $C' = C'(\beta)$ and, therefore, $C = C(\beta)$, by Janson's inequality we have
$$
\Pr[X = 0] \le \Pr[X \le \mu^2 /2 ] \le e^{- \frac{\mu^2}{8 (\mu + \delta)}} \le e^{- \beta n},
$$
as required. This finishes the proof of the lemma.
\end{proof}







% The main tool for proving Connecting Lemma (Lemma \ref{lemma:connecting}) is the criteria for matchings in hypergraphs due to Haxell \cite{H95}. Given a family $\mathcal{E}$ of subsets of some ground set $V$, we denote with $\tau(\mathcal{E})$ the size of a smallest subset $X \subseteq V$ such that $E \cap X \neq \emptyset$ for every $E \in \mathcal{E}$.

% \begin{theorem}(Theorem 3, \cite{H95}) \label{thm:hyp_matching}
% 	Suppose $r \in \mathbb{N}$, and let $\{ H_i = (V, \mathcal{E}_i) \}_{i \in \mathcal{I}}$ be a family of $r$-uniform hypergraphs on the same vertex set. If $\tau(\bigcup_{i \in \mathcal{I}'} \mathcal{E}_i) > (2r - 1)(|\mathcal{I}'| - 1)$ for every $\mathcal{I}' \subseteq \mathcal{I}$, then there exists a family of hyperedges $\{e_i\}_{i \in \mathcal{I}}$ such that $e_i \subseteq \mathcal{E}_i$ and $e_i \cap e_j = \emptyset$ for every $i \neq j \in \mathcal{I}$.
% \end{theorem}

% Note that the statement of Theorem 3 in \cite{H95} is slightly different than Theorem \ref{thm:hyp_matching}. It is easy to see that they are equivalent. Annamalai \cite{annamalai2015finding} recently  gave an algorithm for finding a perfect matching in a bipartite hypergraph satisfying Haxell's condition. Although Annamalai uses the notion of perfect matching in bipartite hypergraphs, one can easily see that the problem studied in \cite{annamalai2015finding} is equivalent to the one of interest to us.  Following the notation of Theorem \ref{thm:hyp_matching}, if $r$ is a fixed constant then the algorithm of Annamalai finds a family of hyperedges $\{e_i\}_{i \in \mathcal{I}}$ such that $e_i \subseteq \mathcal{E}_i$ and $e_i \cap e_j = \emptyset$ for every $i \neq j \in \mathcal{I}$ in time polynomial in the size of the vertex set $V$.
% However, in our application the uniformity of $H_i$'s will be of poly-logarithmic order in the size of $V$ and, thus, we can find the desired family of hyperedges $\{e_i\}_{i \in \mathcal{I}}$  only in time $O(2^{\log^c n})$, where $|V| = n$ and $c > 1$ is a fixed constant.
